Nebular abundance gradient in the Cartwheel galaxy using MUSE data

We here present the results from a detailed analysis of nebular abundances of commonly observed ions in the collisional ring galaxy Cartwheel using the Very Large Telescope (VLT) Multi-Unit Spectroscopic Explorer (MUSE) dataset. The analysis includes 221 HII regions in the star-forming ring, in addition to 40 relatively fainter H$\alpha$ emitting regions in the spokes, disk and the inner ring. The ionic abundances of He, N, O and Fe are obtained using the direct method (DM) for 9, 20, 20, and 17 ring HII regions, respectively, where the S$^{++}$ temperature-sensitive line is detected. For the rest of the regions, including all the nebulae between the inner and the outer ring, we obtained O abundances using the strong-line method (SLM). The ring regions have a median $12+\log\rm{\frac{O}{H}}$=8.19$\pm$0.15, $\log\rm{\frac{N}{O}}=-$1.57$\pm$0.09 and $\log\rm{\frac{Fe}{O}}=-$2.24$\pm$0.09 using the DM. Within the range of O abundances seen in the Cartwheel, the N/O and Fe/O values decrease proportionately with increasing O, suggesting local enrichment of O without corresponding enrichment of primary N and Fe. The O abundances of the disk HII regions obtained using the SLM show a well-defined radial gradient. The mean O abundance of the ring HII regions is lower by $\sim$0.1 dex as compared to the extrapolation of the radial gradient. The observed trends suggest the preservation of the pre-collisional abundance gradient, displacement of most of the processed elements to the ring, as predicted by the recent simulation by Renaud et al. (2018), and post-collisional infall of metal-poor gas in the ring.

==> ReadMe <==
                                                      (Zaragoza-Cardiel+, 2022)
================================================================================================================
Nebular abundance gradient in the Cartwheel galaxy using MUSE data
   Zaragoza-Cardiel J., G\'omez-Gonz\'alez V.M.A., Mayya Y.D.
    =
================================================================================================================
Keywords:  galaxies: star clusters ; galaxies: individual (ESO 350-40 or Cartwheel)


Abstract:
    We here present the results from a detailed analysis of nebular abundances of commonly
    observed ions in the collisional ring galaxy Cartwheel using the Very Large Telescope
    (VLT) Multi-Unit Spectroscopic Explorer (MUSE) dataset. The analysis includes 221 HII 
    regions in the star-forming ring, in addition to 40 relatively fainter emitting regions 
    in the spokes, disk and the inner ring. The ionic abundances of He, N, O and Fe are obtained 
    using the direct method (DM) for 29  ring HII regions where at least one of the NII and SIII 
    temperature-sensitive lines are detected. For the rest of the regions, including all the 
    nebulae between the inner and the outer ring, we obtained O abundances using the strong-line 
    method (SLM). The ring regions have a median 12+log(O/H)=8.13+-0.30,  log(N/O)=-1.6+-0.2 and 
    log(Fe/O)=-2.4+-0.2 using the DM, with the relatively high standard deviation in the O 
    abundance arising due to a systematic azimuthal variation in the derived O abundances in the 
    intense star-forming southern quadrant. The N/O and Fe/O values decrease proportionately 
    with increasing O, suggesting local enrichment of O without corresponding enrichment in N 
    and Fe. The O abundances of the disk HII regions obtained using the SLM show a well-defined 
    radial gradient. The mean O abundance of the ring HII regions is lower by $\sim$0.1~dex as 
    compared to the extrapolation of radial gradient. The observed trends suggest the 
    preservation of the pre-collisional abundance gradient, displacement of most of the 
    processed elements to the ring, as predicted by the recent simulation by Renaud et al. 2018, 
    and post-collisional infall of metal-poor gas in the ring.
    

File Summary:
----------------------------------------------------------------------------------------------------------------
 FileName    Lrecl   Records    Explanations
----------------------------------------------------------------------------------------------------------------
ReadMe           80        .  this file
table_cartwheel 768      252  


----------------------------------------------------------------------------------------------------------------
Byte-by-byte Description of file: table_cartwheel
----------------------------------------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
----------------------------------------------------------------------------------------------------------------
  1-  4   A4     ---       ID             Identification label
  6- 14   F9.7   deg       RAd            Right Ascension (J2000)
 16- 25   F10.6  deg       Decd           Declination (J2000)
 27- 33   F7.1   K         tl             Electron Temperature low ionization
 35- 40   F6.1   K         tl_e           Electron Temperature low ionization error
 42- 48   F7.1   K         th             Electron Temperature high ionization
 50- 55   F6.1   K         th_e           Electron Temperature high ionization error
 57- 63   F7.1   K         tm             Electron Temperature medium ionization
 65- 70   F6.1   K         tm_e           Electron Temperature medium ionization error
 72- 76   F5.1   1/cm3     dens           Electron density from S2 lines
 78- 82   F5.1   1/cm3     dens_e         Electron density error
 84- 90   E7.2   ---       FeIII/H        Abundance of FeIII
 92- 96   E5.1   ---       FeIII/H_e      Abundance of FeIII error
 98-104   E7.2   ---       OI/H           Abundance of OI
106-110   E5.1   ---       OI/H_e         Abundance of OI error
112-118   E7.2   ---       OII/H          Abundance of OII
120-124   E5.1   ---       OII/H_e        Abundance of OII error
126-132   E7.2   ---       OIII/H         Abundance of OIII
134-138   E5.1   ---       OIII/H_e       Abundance of OIII error
140-146   E7.2   ---       NII/H          Abundance of NII
148-152   E5.1   ---       NII/H_e        Abundance of NII error
154-160   F7.3   ---       HeI/H          Abundance of HeI
162-168   F7.3   ---       HeI/H_e        Abundance of HeI error
170-178   F9.5   ---       HeII/H         Abundance of HeII
180-184   E5.1   ---       HeII/H_e       Abundance of HeII error
186-192   E7.2   ---       Fe/H           Abundance of Fe
194-198   E5.1   ---       Fe/H_e         Abundance of Fe error
200-204   E5.1   ---       O/H            Abundance of O
206-210   E5.1   ---       O/H_e          Abundance of O error
212-218   E7.2   ---       N/H            Abundance of N
220-224   E5.1   ---       N/H_e          Abundance of N error
226-232   F7.3   ---       He/H           Abundance of He
234-240   F7.3   ---       He/H_e         Abundance of He error
242-246   F5.1   deg       PA             Position Angle
248-255   F8.3   AA        EW_Ha          Halpha Equivalent width
257-263   F7.3   dex       A_V            Attenuation 
265-271   F7.3   dex       A_V_e          Attenuation error
273-277   F5.1   kpc       radius         Galactrocentric radius
279-286   F8.4   dex       12+log(O/H)s   Oxygen abundance derived with the strong lines method
288-295   F8.4   dex       12+log(O/H)s_e Oxygen abundance error derived with the strong lines method
297-303   F7.3   AA        EW_Hb          Hbeta Equivalent width
305-309   F5.1   ---       SNR_Hb         SNR of Hb flux
311-319   E9.4   erg/s/cm2 H1r_4861A      Attenuation-corrected flux of H1r_4861A
321-325   E5.1   erg/s/cm2 H1r_4861A_e    H1r_4861A error
327-332   F6.2   ---       Fe3_4659A      100*Fe3_4659A/H1r_4861A
334-339   F6.2   ---       Fe3_4659A_e    100*Fe3_4659A/H1r_4861A error
341-346   F6.2   ---       He2r_4686A     100*He2r_4686A/H1r_4861A
348-353   F6.2   ---       He2r_4686A_e   100*He2r_4686A/H1r_4861A error
355-359   F5.1   ---       Fe3_4701A      100*Fe3_4701A/H1r_4861A
361-366   F6.2   ---       Fe3_4701A_e    100*Fe3_4701A/H1r_4861A error
368-373   F6.2   ---       Ar4_4711A      100*Ar4_4711A/H1r_4861A
375-380   F6.2   ---       Ar4_4711A_e    100*Ar4_4711A/H1r_4861A error
382-387   F6.2   ---       Ar4_4740A      100*Ar4_4740A/H1r_4861A
389-394   F6.2   ---       Ar4_4740A_e    100*Ar4_4740A/H1r_4861A error
396-401   F6.2   ---       He1r_4922A     100*He1r_4922A/H1r_4861A
403-408   F6.2   ---       He1r_4922A_e   100*He1r_4922A/H1r_4861A error
410-416   F7.3   ---       O3_4959A       100*O3_4959A/H1r_4861A
418-422   E5.1   ---       O3_4959A_e     100*O3_4959A/H1r_4861A error
424-429   F6.2   ---       Fe3_4986A      100*Fe3_4986A/H1r_4861A
431-436   F6.2   ---       Fe3_4986A_e    100*Fe3_4986A/H1r_4861A error
438-444   F7.3   ---       O3_5007A       100*O3_5007A/H1r_4861A
446-453   F8.4   ---       O3_5007A_e     100*O3_5007A/H1r_4861A error
455-461   F7.3   ---       He1r_5016A     100*He1r_5016A/H1r_4861A
463-469   F7.3   ---       He1r_5016A_e   100*He1r_5016A/H1r_4861A error
471-475   F5.1   ---       He1r_5048A     100*He1r_5048A/H1r_4861A
477-482   F6.2   ---       He1r_5048A_e   100*He1r_5048A/H1r_4861A error
484-488   F5.1   ---       Fe3_5270A      100*Fe3_5270A/H1r_4861A
490-495   F6.2   ---       Fe3_5270A_e    100*Fe3_5270A/H1r_4861A error
497-502   F6.2   ---       N2_5755A       100*N2_5755A/H1r_4861A
504-509   F6.2   ---       N2_5755A_e     100*N2_5755A/H1r_4861A error
511-517   F7.3   ---       He1r_5876A     100*He1r_5876A/H1r_4861A
519-525   F7.3   ---       He1r_5876A_e   100*He1r_5876A/H1r_4861A error
527-533   F7.3   ---       O1_6300A       100*O1_6300A/H1r_4861A
535-541   F7.3   ---       O1_6300A_e     100*O1_6300A/H1r_4861A error
543-549   F7.3   ---       S3_6312A       100*S3_6312A/H1r_4861A
551-557   F7.3   ---       S3_6312A_e     100*S3_6312A/H1r_4861A error
559-564   F6.2   ---       O1_6364A       100*O1_6364A/H1r_4861A
566-571   F6.2   ---       O1_6364A_e     100*O1_6364A/H1r_4861A error
573-579   F7.3   ---       N2_6548A       100*N2_6548A/H1r_4861A
581-588   F8.4   ---       N2_6548A_e     100*N2_6548A/H1r_4861A error
590-595   F6.2   ---       H1r_6563A      100*H1r_6563A/H1r_4861A
597-604   F8.4   ---       H1r_6563A_e    100*H1r_6563A/H1r_4861A error
606-612   F7.3   ---       N2_6584A       100*N2_6584A/H1r_4861A
614-621   F8.4   ---       N2_6584A_e     100*N2_6584A/H1r_4861A error
623-629   F7.3   ---       He1r_6678A     100*He1r_6678A/H1r_4861A
631-637   F7.3   ---       He1r_6678A_e   100*He1r_6678A/H1r_4861A error
639-645   F7.3   ---       S2_6716A       100*S2_6716A/H1r_4861A
647-651   E5.1   ---       S2_6716A_e     100*S2_6716A/H1r_4861A error
653-659   F7.3   ---       S2_6731A       100*S2_6731A/H1r_4861A
661-668   F8.4   ---       S2_6731A_e     100*S2_6731A/H1r_4861A error
670-676   F7.3   ---       He1r_7065A     100*He1r_7065A/H1r_4861A
678-684   F7.3   ---       He1r_7065A_e   100*He1r_7065A/H1r_4861A error
686-690   F5.1   ---       He1r_7281A     100*He1r_7281A/H1r_4861A
692-696   F5.1   ---       He1r_7281A_e   100*He1r_7281A/H1r_4861A error
698-703   F6.2   ---       O2_7319A       100*O2_7319A/H1r_4861A
705-710   F6.2   ---       O2_7319A_e     100*O2_7319A/H1r_4861A error
712-717   F6.2   ---       O2_7330A       100*O2_7330A/H1r_4861A
719-724   F6.2   ---       O2_7330A_e     100*O2_7330A/H1r_4861A error
726-731   F6.2   ---       Ar3_7751A      100*Ar3_7751A/H1r_4861A
733-738   F6.2   ---       Ar3_7751A_e    100*Ar3_7751A/H1r_4861A error
740-745   F6.2   ---       O1_8446A       100*O1_8446A/H1r_4861A
747-752   F6.2   ---       O1_8446A_e     100*O1_8446A/H1r_4861A error
754-760   F7.3   ---       S3_9069A       100*S3_9069A/H1r_4861A
762-768   F7.3   ---       S3_9069A_e     100*S3_9069A/H1r_4861A error

----------------------------------------------------------------------------------------------------------------

Acknowledgements:
   Javier Zaragoza-Cardiel, javier.zaragoza(at)inaoep.mx

================================================================================================================
     (prepared by author  / pyreadme )

